Analytical Heterogeneous Die-to-Die 3D Placement with Macros

This paper presents an innovative approach to 3D mixed-size placement in heterogeneous face-to-face (F2F) bonded 3D ICs. We propose an analytical framework that utilizes a dedicated density model and a bistratal wirelength model, effectively handling macros and standard cells in a 3D solution space. A novel 3D preconditioner is developed to resolve the topological and physical gap between macros and standard cells. Additionally, we propose a mixed-integer linear programming (MILP) formulation for macro rotation to optimize wirelength. Our framework is implemented with full-scale GPU acceleration, leveraging an adaptive 3D density accumulation algorithm and an incremental wirelength gradient algorithm. Experimental results on ICCAD 2023 contest benchmarks demonstrate that our framework can achieve 5.9% quality score improvement compared to the first-place winner with 4.0x runtime speedup. Additional experiments on modern RISC-V designs further validate the generalizability and superiority of our framework.

==> doc/bio.tex <==

\vspace{-.4in}
\begin{IEEEbiography}[{\includegraphics[height=1.24in,clip,keepaspectratio]{./avatar/yxzhao}}]{Yuxuan Zhao}
    received the B.S. degree in Information Engineering from Zhejiang University in 2021. He is currently pursuing his Ph.D. degree at the Department of Computer Science and Engineering, The Chinese University of Hong Kong. His current research interests include high performance computing in physical design and machine learning in EDA.
\end{IEEEbiography}
\vspace{-.4in}
\begin{IEEEbiography}[{\includegraphics[height=1.24in,clip,keepaspectratio]{./avatar/pyliao}}]{Peiyu Liao}
    received the B.S. degree from the School of Mathematical Sciences, Zhejiang University in 2017, and the M.S. degree from the School of Engineering, The Hong Kong University of Science and Technology in 2019. He is currently pursuing his Ph.D. degree at the Department of Computer Science and Engineering, The Chinese University of Hong Kong. His current research interests include high performance computing and numerical optimization in physical design.
\end{IEEEbiography}
\vspace{-.4in}
\begin{IEEEbiography}[{\includegraphics[height=1.24in,clip,keepaspectratio]{./avatar/stliu}}]{Siting Liu}
    received her B.S. degree from the Department of Computer Science, Huazhong University of Science and Technology in 2020. She is currently pursuing her Ph.D. degree at the Department of Computer Science and Engineering, The Chinese University of Hong Kong. She is a visiting student at the School of Integrated Circuits, Peking University. \\ Her current research interests include deep learning applications and GPU acceleration in physical design. Ms. Liu received Best Paper Award from DATE 2022, and Best Paper Award Nomination from DATE 2021.
    \end{IEEEbiography}
\vspace{-.4in}
\begin{IEEEbiography}[{\includegraphics[height=1.24in,clip,keepaspectratio]{./avatar/jxjiang}}]{Jiaxi Jiang}
    received his B.E. degree in Computer Science from Northwestern Polytechnical University in 2023. He is currently pursuing his Ph.D. degree at the Department of Computer Science and Engineering, The Chinese University of Hong Kong. His current research interests include physical design, machine learning applications in EDA.
\end{IEEEbiography}
\vspace{-.4in}
\begin{IEEEbiography}[{\includegraphics[height=1.24in,clip,keepaspectratio]{./avatar/ylin}}]{Yibo Lin}
    (M’19) received the B.S. degree in Microelectronics from Shanghai Jiaotong University in 2013. He obtained his Ph.D. degree in Electrical and Computer Engineering from the University of Texas at Austin in 2018 advised by Prof. David Z. Pan. He worked as a postdoctoral researcher at the University of Texas at Austin from 2018 to 2019. He currently is an assistant professor in the School of Integrated Circuits at Peking University. His research interests include physical design, machine learning applications, and heterogeneous computing in VLSI CAD. He is a recipient of the Best Paper Awards at preimier EDA/CAD journals/conferences like TCAD, DAC, DATE, ISPD, etc.
    \end{IEEEbiography}
\vspace{-.4in}
\begin{IEEEbiography}[{\includegraphics[height=1.26in,clip,keepaspectratio]{./avatar/byu}}]
    {Bei Yu}
    (M'15-SM'22)
    received the Ph.D.~degree from The University of Texas at Austin in 2014.
    He is currently an Associate Professor in the Department of Computer Science and Engineering, The Chinese University of Hong Kong.
    He has served as TPC Chair of ACM/IEEE Workshop on Machine Learning for CAD, and in many journal editorial boards and conference committees.
    He is Editor of IEEE TCCPS Newsletter.
    He received ten Best Paper Awards from IEEE TSM 2022, DATE 2022, ICCAD 2021 \& 2013, ASPDAC 2021 \& 2012, ICTAI 2019, Integration, the VLSI Journal in 2018,
    ISPD 2017, SPIE Advanced Lithography Conference 2016, and six ICCAD/ISPD contest awards.
\end{IEEEbiography}


